Combining p-multigrid and multigrid reduced in time methods to obtain a scalable solver for Isogeometric Analysis

Isogeometric Analysis (IgA) has become a viable alternative to the Finite Element Method (FEM) and is typically combined with a time integration scheme within the method of lines for time-dependent problems. However, due to a stagnation of processors clock speeds, traditional (i.e. sequential) time integration schemes become more and more the bottleneck within these large-scale computations, which lead to the development of parallel-in-time methods like the Multigrid Reduced in Time (MGRIT) method. Recently, MGRIT has been succesfully applied by the authors in the context of IgA showing convergence independent of the mesh width, approximation order of the B-spline basis functions and time step size for a variety of benchmark problems. However, a strong dependency of the CPU times on the approximation order was visible when a standard Conjugate Gradient method was adopted for the spatial solves within MGRIT. In this paper we combine MGRIT with a state-of the-art solver (i.e. a p-multigrid method), specifically designed for IgA, thereby significantly reducing the overall computational costs of MGRIT. Furthermore, we investigate the performance of MGRIT and its scalability on modern copmuter architectures.

==> Comments <==
// Commented out of the paper


\begin{comment}
\section{Numerical results (Dirichlet)}
\label{sec:results}

To assess the quality of the MGRIT method when applied in combination with Isogeometric Analysis, we consider the time-dependent heat equation in two dimensions given by Equation \eqref{eq:heat}. Based on a spatial discretization with B-spline basis functions of order $p$ and mesh width $h$, Backward Euler or Forward Euler is applied for the time discretization. In particular, we explore the influence of the number of levels, cycle type and accuracy of the spatial solves on the number of MGRIT iterations. Furthermore, we investigate the parallel performance of MGRIT and compare its efficiency with sequential time stepping methods.

The open-source C++ library G+Smo \cite{gismo} is used to discretize the model problem in space, while, for the MGRIT algorithm, the parallel-in-time code XBraid, developed at Lawrence Livermore National Lab, is adopted \cite{xbraid}.   


As a model problem, we solve Equation \eqref{eq:heat} on the time domain $T=[0,0.1]$ with $\kappa =1$. Furthermore, the righthandside is chosen equal to one and the initial condition is equal to zero. This initial condition is chosen as well as initial guess at all times $t>0$. The MGRIT method is said to have reached convergence if the residual at the end of an iteration is smaller or equal to $10^{-10}$, unless stated otherwise.

The domain $\Omega$ is varied for the different model problems: For the first model problem, referred to as MP-1, we consider the unit square (i.e. $\Omega = [0,1]^2$). As Isogeometric Analysis describes curved geometries more accurately compared to FEM, the second model involves a curved geometry. That is, as MP-2, $\Omega$ is chosen to be a quarter annulus defined in the first quadrant with inner radius of $1$ and an outer radius of $2$. Finally, a multipatch geometry is considered as MP-3. Figure \ref{fig:domain} illustrates the considered spatial domains for all model problems.


\begin{figure}
\begin{tikzpicture}[scale=0.7]
\draw (0,0) -- (4,0) -- (4,4) -- (0,4) -- (0,0);

\draw (8,0) -- (10,0);
\draw (6,4) -- (6,2);
\draw (10,0) arc (0:90:4cm);
\draw (8,0) arc (0:90:2cm);

\draw[dashed] (14,0) -- (14,4);
\draw[dashed] (12,2) -- (16,2);
\draw (12,0) -- (16,0) -- (16,4) -- (12,4) -- (12,0);
\end{tikzpicture}
\caption{Spatial domain $\Omega$ for the model problems MP-1, MP-2 and MP-3.}
\label{fig:domain}
\end{figure}

\subsection*{Implicit time integration}

First, we consider the MGRIT method using both V-cycles and F-cycles for the implicit case (i.e. Backward Euler). At each time step, a linear system of equations has to be solved, which is done by means of a Conjugate Gradient method. Table \ref{tab:1} shows the number of MGRIT iterations for different mesh widths $h$ and approximation orders $p$ of the B-spline basis functions when a two-level method is considered. Here, F-relaxation is applied at all grids of the MGRIT hierarchy. The number of time steps for all configurations equals $100$.

As a two-level method is considered, the number of iterations obtained when considering $V$-cycles is equal to the use of $F$-cycles for all configurations. Furthermore, the number of iterations is constant for all values of $h$, implying MGRIT to be an optimal algorithm with respect to the problem size. For increasing values of $p$, we observe that the number of MGRIT iterations is constant. This is of particular interest, as the convergence rate of standard multigrid methods is known to be dependent on the approximation order $p$ \cite{Gahalaut2013}.  


\begin{table}[h]
\begin{tabular}{c|cccc|cccc|}
  \multicolumn{1}{c|}{}   & \multicolumn{4}{c|}{$V$-cycle}   & \multicolumn{4}{c|}{$F$-cycle}    \\  
						 & $p=2$ & $p=3$ & $p=4$ & $p=5$ & $p=2$ & $p=3$ & $p=4$ & $p=5$  \\ \hline
		$h=2^{-4}$		 & 	$6$	 & $6$	 & $6$   & 	$7$  &  $6$  & 	$6$	 & 	$6$  &   $7$     \\
		$h=2^{-5}$		 & 	$7$	 & $7$	 & $7$	 & 	$7$  &  $7$  & 	$7$	 & 	$7$  &   $7$     \\
		$h=2^{-6}$		 & 	$7$	 & $7$	 & $7$	 & 	$7$  &  $7$  & 	$7$	 & 	$7$  &   $7$     \\
		$h=2^{-7}$		 & 	$7$	 & $7$	 & $7$	 & 	$7$  &  $7$  & 	$7$	 & 	$7$  &   $7$     \\
\end{tabular}
\caption{Number of two-level MGRIT iterations for solving the model problem when adopting $V$-cycle or $F$-cycles.}
\label{tab:1}
\end{table}

Alternatively, a multilevel MGRIT method can be applied as well. Here coarsening is applied with coarsening factor $m=2$, leading to a hierarchy consisting of five levels $(L=5)$. Table \ref{tab:2} shows the number of MGRIT iterations when either $V$-cycles or $F$-cycles are adopted within MGRIT. For all configurations, the use of an $F$-cycle leads to a lower number of MGRIT iterations to reach convergence. However, it should be noted that the computational costs of an $F$-cycle is higher compared to a $V$-cycle. In the next Section, a weak scalability study is preformed using both cycle types.    

\begin{table}[h]
\begin{tabular}{c|cccc|cccc|}
  \multicolumn{1}{c|}{}   & \multicolumn{4}{c|}{$V$-cycle}   & \multicolumn{4}{c|}{$F$-cycle}    \\  
						& $p=2$ & $p=3$ & $p=4$ & $p=5$ & $p=2$ & $p=3$ & $p=4$ & $p=5$  \\ \hline
		$h=2^{-4}$		& 	$8[29]$	 & 	$8[50]$	 &  $8[62]$   & $8[126]$	 &   $7$ & $7$	 & $7$	 &  $7$   \\
		$h=2^{-5}$		& 	$8[28]$	 & 	$8[63]$	 & 	$8[111]$  & $8[235]$	 &   $7$ & $7$	 & $7$	 &  $7$   \\
		$h=2^{-6}$		& 	$8[36]$	 & 	$8[63]$	 & 	$8[125]$  & $8[290]$	 &   $7$ & $7$	 & $7$   &  $7$   \\
		$h=2^{-7}$		& 	$9[76]$	 & 	$9[69]$	 & 	$9[130]$  & $9[290]$	 &   $7$ & $7$	 & $7$	 &  $7$    \\
\end{tabular}
\caption{Number of multilevel MGRIT iterations for solving the model problem when adopting $V$-cycle or $F$-cycles.}
\label{tab:2}
\end{table}

Apart the mesh width, the size of the linear system given by Equation \eqref{eq:mgrit} is influenced by the time step size. Furthermore, with MGRIT, coarsening is applied in $\Delta t$, instead of the mesh width (as with 'standard' multigrid methods). Therefore, it's interesting to investigate the influence of the time step size (or equivalently the number of time steps with a fixed end time $T$) on the number of MGRIT iterations. Table \ref{tab:2A} shows the number of multilevel MGRIT iterations for different time step sizes. Here, $V$-cycles and a constant mesh width of $h=2^{-6}$ are considered for all configurations. Clearly, the number of MGRIT iterations is independent of the time step size for all values of the approximation order $p$. 

\begin{table}[h]
\centering
\begin{tabular}{c|cccc}
						& $p=2$ & $p=3$ & $p=4$ & $p=5$     \\ \hline
		$N_t = 50$		& 	$8$	 & 	$8$	 &  $8$  & $8$	    \\
		$N_t =100$		& 	$8$	 & 	$8$	 & 	$8$  & $8$	    \\
		$N_t =200$		& 	$9$	 & 	$9$	 & 	$9$  & $9$	    \\
		$N_t =400$		& 	$9$	 & 	$9$	 & 	$9$  & $9$	    \\
\end{tabular}
\caption{Number of multilevel MGRIT iterations (using $V$-cycles) for solving MP-1 for a different number of time steps and $h=2^{-6}$.}
\label{tab:2A}
\end{table}

With implicit time integration methods, spatial solves are required at every time step denoted by the function $\Psi$. As these linear systems are solved by means of an iterative method (e.g. Conjugate Gradient), the adopted stopping criterion in these methods (at the coarser levels) might influence the overall convergence of the MGRIT method.   

Table \ref{tab:3} shows the number of MGRIT iterations for different values of the stopping criterion at the coarse levels of the MGRIT hierarchy. Here, $\epsilon$ denotes the norm of the residual divided by the norm of the righthandside and a mesh width is adopted of $h=2^{-6}$. In general, the number of MGRIT is independent of the chosen stopping criterion on the coarser levels. However, when the stopping criterion is chosen too small, the number of MGRIT increases significantly, in particular for smaller values of $p$. 

\begin{table}[h]
\centering
\begin{tabular}{c|cccc}
						& $p=2$ & $p=3$ & $p=4$ & $p=5$  \\ \hline
$\epsilon=10^{-6}$		& 	$*$	 & 	$14$ &  $11$ & $10$	 \\
$\epsilon=10^{-8}$		& 	$8$	 & 	$8$	 & 	$9$  & $8$	 \\
$\epsilon=10^{-10}$		& 	$8$	 & 	$8$	 & 	$8$  & $8$   \\
$\epsilon\approx10^{-16}$& 	$8$	 & 	$8$	 & 	$8$  & $8$   \\
\end{tabular}
\caption{Number of multilevel MGRIT iterations for solving the model problem (using $V$-cycles) when adopting different stopping criteria at the coarse levels.}
\label{tab:3}
\end{table}

\subsection*{Explicit time integration schemes}
The use of explicit time integration schemes in the context of parallel-in-time integration is on one hand highly relevant, as the required number of time steps needed to ensure stability is relatively high. On the other hand, coarsening with respect to the time step size might still exhibit stability issues at coarser levels. Therefore, explicit-implicit methods are often considered, where explicit time integration is applied on the fine scale problem, while implicit methods are adopted at the coarser levels. 

An obvious drawback of this approach is that one has to implement both time integration schemes within the code. Furthermore, the question remains to which extend the resulting MGRIT algorithm remains robust in the mesh width and/or approximation order. Table \ref{tab:3A} shows the number of two-level MGRIT iterations for different number of time steps when adopting a mesh width of $h=2^{-6}$. Here, explicit Euler is applied at the fine level, while Backward Euler is applied at the coarse level. Note that, provided a small enough time step size is chosen, the resulting MGRIT method convergences is a relatively low number of iterations. However, the higher the approximation order, the lower the time step size has to be chosen to ensure convergence of the MGRIT method. 

\begin{table}[h]
\centering
\begin{tabular}{c|cccc}
				& $p=2$ & $p=3$ & $p=4$  & $p=5$  \\ \hline
$N_t=200$		& 	$*$	 & 	$*$  &  $*$  & $*$	 \\
$N_t=400$		& 	$10$ & 	$22$ & 	$*$  & $*$	 \\
$N_t=600$		& 	$10$ & 	$10$ & 	$*$  & $*$   \\
$N_t=800$		& 	$9$	 & 	$9$	 & 	$10$ & $*$   \\
\end{tabular}
\caption{Number of two-level MGRIT iterations for solving the model problem (using $V$-cycles) when adopting a different number of time steps. Here, explicit Euler is applied at the fine level, while Backward Euler is applied at the coarse level.}
\label{tab:3A}
\end{table}

Apart from first order time integration methods, MGRIT can be combined with higher-order time integration methods as well. Table \ref{tab:3B} shows the number of two-level MGRIT iterations when the second-order accurate Crank-Nicolson method is applied for the time integration when adopting a mesh width of $h=2^{-6}$. The resulting MGRIT method convergences is a relatively low number of iterations, provided a small enough time step size is chosen.

\begin{table}[h]
\centering
\begin{tabular}{c|cccc}
				& $p=2$ & $p=3$ & $p=4$  & $p=5$  \\ \hline
$N_t=200$		& 	$5$	 & 	$8$  &  $36$ & $*$	 \\
$N_t=400$		& 	$4$  & 	$4$  & 	$6$  & $20$	 \\
$N_t=600$		& 	$4$  & 	$4$  & 	$4$  & $6$   \\
$N_t=800$		& 	$4$	 & 	$4$	 & 	$4$  & $4$   \\
\end{tabular}
\caption{Number of two-level MGRIT iterations for solving the model problem (using $V$-cycles) when adopting a different number of time steps. Here, Crank-Nicolson is applied at all levels.}
\label{tab:3B}
\end{table}

\subsection*{Alternative model problems}

In this section, we consider the MGRIT method applied on curved and multipatch geometries (while using Backward-Euler). Table \ref{tab:4} shows the number of two-level and multilevel MGRIT iterations needed to reach convergence for the heat equation on a quarter annulus (i.e. MP-2). Here, $V$-cycles are applied and results can be compared to Table \ref{tab:1} and \ref{tab:2}. In general, results are very similar to the ones obtained for MP-1, showing iteration numbers indepedent of the problem size and order of the B-spline basis functions.


\begin{table}[h]
\begin{tabular}{c|cccc|cccc|}
  \multicolumn{1}{c|}{}   & \multicolumn{4}{c|}{two-level}   & \multicolumn{4}{c|}{multilevel}    \\  
						 & $p=2$ & $p=3$ & $p=4$ & $p=5$ & $p=2$ & $p=3$ & $p=4$ & $p=5$  \\ \hline
		$h=2^{-4}$		 & 	$7$	 & $7$	 & $7$   & 	$7$  &  $8$  & 	$8$	 & 	$8$  &   $8$     \\
		$h=2^{-5}$		 & 	$7$	 & $7$	 & $7$	 & 	$7$  &  $8$  & 	$8$	 & 	$8$  &   $8$     \\
		$h=2^{-6}$		 & 	$7$	 & $7$	 & $7$	 & 	$7$  &  $8$  & 	$8$	 & 	$8$  &   $8$     \\
		$h=2^{-7}$		 & 	$7$	 & $7$	 & $7$	 & 	$7$  &  $9$  & 	$9$	 & 	$9$  &   $?$     \\
\end{tabular}
\caption{Number of two-level or multilevel MGRIT iterations for solving MP-2 when adopting $V$-cycles.}
\label{tab:4}
\end{table}

As a third model problem, we consider $\Omega=[0,1]^2$, which can be described by a single mapping and split it unformly in both directions. Table \ref{tab:5} shows the number of iterations needed for a multipatch geometry. The results are very similar to those obtained for MP-1 and MP-2.  

\begin{table}[h]
\begin{tabular}{c|cccc|cccc|}
  \multicolumn{1}{c|}{}   & \multicolumn{4}{c|}{two-level}   & \multicolumn{4}{c|}{multilevel}    \\  
						 & $p=2$ & $p=3$ & $p=4$ & $p=5$ & $p=2$ & $p=3$ & $p=4$ & $p=5$  \\ \hline
		$h=2^{-4}$		 & 	$6$	 & $7$	 & $7$   & 	$7$  &  $8$  & 	$8$	 & 	$8$  &   $8$     \\
		$h=2^{-5}$		 & 	$7$	 & $7$	 & $7$	 & 	$7$  &  $8$  & 	$8$	 & 	$8$  &   $8$     \\
		$h=2^{-6}$		 & 	$7$	 & $7$	 & $7$	 & 	$7$  &  $8$  & 	$8$	 & 	$8$  &   $8$     \\
		$h=2^{-7}$		 & 	$7$	 & $7$	 & $7$	 & 	$7$  &  $9$  & 	$9$	 & 	$9$  &   $9$     \\
\end{tabular}
\caption{Number of two-level or multilevel MGRIT iterations for solving MP-3 when adopting $V$-cycles.}
\label{tab:5}
\end{table}

As in the previous Section, the number of MGRIT iterations can be determined for different time step sizes as well. Table \ref{tab:5A} shows the number of multilevel MGRIT $V$-cycles needed to reach convergence for MP-2 and MP-3 for different values of the time step size. 

\begin{table}[h]
\begin{tabular}{l|cccc|cccc|}
  \multicolumn{1}{c|}{}   & \multicolumn{4}{c|}{MP-2}   & \multicolumn{4}{c|}{MP-3}    \\  
						 & $p=2$ & $p=3$ & $p=4$ & $p=5$ & $p=2$ & $p=3$ & $p=4$ & $p=5$  \\ \hline
		$N_t =50$		 & 	$8$	 & $8$	 & $8$   & 	$8$  &  $8$  & 	$8$	 & 	$8$  &   $8$     \\
		$N_t =100$		 & 	$8$	 & $8$	 & $8$	 & 	$8$  &  $8$  & 	$8$	 & 	$8$  &   $8$     \\
		$N_t =200$		 & 	$9$	 & $9$	 & $9$	 & 	$9$  &  $9$  & 	$9$	 & 	$9$  &   $9$     \\
		$N_t =400$		 & 	$9$	 & $9$	 & $9$	 & 	$9$  &  $9$  & 	$9$	 & 	$9$  &   $9$     \\
\end{tabular}
\caption{Number of multilevel MGRIT iterations for solving MP-2 and MP-3 when adopting $V$-cycles.}
\label{tab:5A}
\end{table}

\newpage

\subsection*{Parallel performance}

To investigate the parellel performance of the MGRIT algorithm, we consider MP-1 for a different number of processors. Here, we consider a traditional backward-Euler time stepping method to the (multilevel) MGRIT method. For the MGRIT method, $V$-cycles are adopted. Figure \ref{fig:parallel} shows the CPU timings of the MGRIT method for a different number of processors. Clearly, increasing the number of processors significantly decreases the CPU times. However, compared to a sequential time integration method, the timings are relatively high.  

\begin{figure}[h!]
\centering
  \begin{tikzpicture}[scale=1.0]
    \begin{axis}[nodes near coords={\pgfmathprintnumber[fixed,fixed zerofill,precision=0]{\pgfplotspointmeta}},point meta=rawy,ybar,every node near coord/.append style={rotate=90, anchor=west,font=\tiny},legend columns=1,legend pos=north west, xmin= 0,xmax=30,ymode=log,ymin=1,ymax=10000,ylabel=CPU Time (s),line width=0.25pt,bar width=0.2cm,bar shift=8mm,xticklabels=\emptynodes]
       \addplot[fill=blue!40] plot coordinates 
      {
        (1,    4.06)
        (7,    12.85)
        (13,   37.34)
        (19,   126.16)
       };
      \addlegendentry{B-Euler}
       \addplot[fill=orange!40] plot coordinates 
      {
        (2,    139.94) %144.0)
        (8,    371.88)%384.73)
        (14,   986.40)%1023.74)
        (20,   3005.13)%3131.29)
        
       };
      \addlegendentry{$MGRIT_1$}
       \addplot[fill=green!40] plot coordinates 
      {
        (3,    77.01)%81.07)
        (9,    234.81)%247.66)
        (15,   633.22)%670.56)
        (21,   1822.11)%1948.27)
       };
      \addlegendentry{$MGRIT_2$}
      \addplot[fill=red!40] plot coordinates 
      {
        (4,    52.09)%56.15)
        (10,   159.01)%171.86)
        (16,   412.45)%449.79)
        (22,   1187.57)%1313.73)
        };
      \addlegendentry{$MGRIT_4$}
      \end{axis}
        \draw (1.35,-0.45)  node{$p=2$};
        \draw (2.74,-0.45)  node{$p=3$};
        \draw (4.13,-0.45)  node{$p=4$};
        \draw (5.52,-0.45)  node{$p=5$};
\end{tikzpicture}
\caption{CPU times for MGRIT and a sequential algorithm for a different number of processors and a fixed problem size ($h=2^{-6},N_t=100$).}
\label{fig:parallel}
\end{figure}

Alternatively, the CPU times can be investigated when the size per processor is kept constant. Figure \ref{fig:weak_parallel} shows the CPU times for both a sequential time integration scheme and MGRIT. For both methods, the computational time increases with the number of processors (and the larger the total problem size). However, relatively seen the CPU times grow significantly slower for the MGRIT method. As the number of processors available equals only $4$, the sequential time integration method outperforms the MGRIT method for all settings.


\begin{figure}[h!]
\centering
  \begin{tikzpicture}[scale=1.0]
    \begin{axis}[nodes near coords={\pgfmathprintnumber[fixed,fixed zerofill,precision=1]{\pgfplotspointmeta}},point meta=rawy,ybar,every node near coord/.append style={rotate=90, anchor=west,font=\tiny},legend columns=1,legend pos=north west, xmin= 0,xmax=30,ymode=log,ymin=1,ymax=5000,ylabel=CPU Time (s),line width=0.25pt,bar width=0.2cm,bar shift=8mm,xticklabels=\emptynodes]
       \addplot[fill=blue!40] plot coordinates 
      {
        (1,    0.88)
        (7,    2.64)
        (13,   5.60)
        (19,   15.19)
       };
      \addlegendentry{$BE_1$}
       \addplot[fill=orange!40] plot coordinates 
      {
        (2,    4.11)
        (8,    12.99)
        (14,   37.73)
        (20,   127.54)
        
       };
      \addlegendentry{$BE_4$}
       \addplot[fill=green!40] plot coordinates 
      {
        (3,    32.11)%32.99)
        (9,    85.14)%87.78)
        (15,   186.46)%192.06)
        (21,   534.48)%549.67)
       };
      \addlegendentry{$MGRIT_1$}
      \addplot[fill=red!40] plot coordinates 
      {
        (4,    52.06)%56.17)
        (10,   158.89)%171.88)
        (16,   412.43)%450.16)
        (22,   1187.00)%1314.54)
        };
      \addlegendentry{$MGRIT_4$}
      \end{axis}
        \draw (1.35,-0.45)  node{$p=2$};
        \draw (2.74,-0.45)  node{$p=3$};
        \draw (4.13,-0.45)  node{$p=4$};
        \draw (5.52,-0.45)  node{$p=5$};
\end{tikzpicture}
\caption{CPU times for MGRIT and a sequential algorithm for a fixed problem size per processor ($N_t=100$).}
\label{fig:weak_parallel}
\end{figure}

Next, we consider a node on the DIAM cluster (node 6), allowing us to obtain results up to $8$ processors. Figure \ref{fig:paralleltype} shows the strong scaling for different cycle types of the MGRIT method compared to a sequential algorithm. Clearly, for the configurations, the use of a two-level method is significantly faster compared to a multilevel method for all configurations. Furthermore, even though the number of iterations is higher, the use of a $V$-cycle leads (overall) to a faster numerical method compared to the use of $F$-cycles. Finally, it should be emphasized that increasing the number of processors from $4$ to $8$ doesn't lead to a significant reduction in CPU time. 

\begin{figure}
\centering
   \begin{tikzpicture}[scale=1.0]
    \begin{axis}[xlabel=Number of processors,ylabel=CPU Time (s),legend pos = north east, legend columns = 1,legend cell align={left}]
       \addplot[blue,mark=*] plot coordinates 
      {
        (1,    15.92)
        (2,    15.88)
        (4,    15.82)
        (8,    16.55)
        };
      \addlegendentry{Sequential}
      \addplot[red,mark=*] plot coordinates 
      {
        (1,    576.58)%592.50)
        (2,    330.06)%345.94)
        (4,    219.85)%235.67)
        (8,    219.04)%235.59)
        };
      \addlegendentry{V-cycle} 
      \addplot[orange,mark=*] plot coordinates 
      {
        (1,    868.77)%884.69)
        (2,    495.44)%511.32)
        (4,    331.36)%347.18)
        (8,    328.87)%345.42)
        };
      \addlegendentry{F-cycle} 
      \addplot[green,mark=*] plot coordinates 
      {
        (1,    227.19)%234.11)
        (2,    147.96)%163.84)
        (4,    107.03)%122.85)
        (8,    105.07)%121.62)
        };
      \addlegendentry{Two-level} 
      \end{axis}
\end{tikzpicture}
\caption{CPU times for different variants of MGRIT and a sequential algorithm for a fixed problem size ($h=2^{-7},p=2$).}
\label{fig:paralleltype}
\end{figure}

Finally, we investigate the strong scalability of two-level MGRIT method for different refinement levels. Figure \ref{fig:parallelrefinement} shows results with the two-level MGRIT algorithm, which was shown to be the most MGRIT method for these configurations. For all refinement levels, however, the speed-up obtained when going from $4$ to $8$ processors is limited. 


\begin{figure}
\centering
   \begin{tikzpicture}[scale=1.0]
    \begin{axis}[xlabel=Number of processors,ylabel=CPU Time (s),ymode=log,ymax=10000,legend pos = north east, legend columns = 3,legend cell align={left}]
       \addplot[blue,mark=*] plot coordinates 
      {
        (1,    47.97)%51.44)
        (2,    30.88)%34.35)
        (4,    20.27)%23.73)
        (8,    18.32)%21.81)
        };
      \addlegendentry{$h=2^{-6}$}
      \addplot[blue,mark=o] plot coordinates 
      {
        (1,    3.47)
        (2,    3.47)
        (4,    3.46)
        (8,    3.49)
        };
      \addlegendentry{$h=2^{-6}$}
      \addplot[red,mark=*] plot coordinates 
      {
        (1,    216.68)%232.62)
        (2,    147.75)%163.80)
        (4,    106.97)%122.81)
        (8,    105.02)%122.20)
        };
      \addlegendentry{$h=2^{-7}$} 
       \addplot[red,mark=o] plot coordinates 
      {
        (1,    15.94)
        (2,    16.05)
        (4,    15.84)
        (8,    17.18)
        };
      \addlegendentry{$h=2^{-7}$} 
      \addplot[orange,mark=*] plot coordinates 
      {
        (1,    991.15)%1069.39)
        (2,    689.58)%766.03)
        (4,    529.16)%607.87)
        (8,    509.58)%601.74)
        };
      \addlegendentry{$h=2^{-8}$}
      \addplot[orange,mark=o] plot coordinates 
      {
        (1,    78.24)
        (2,    76.45)
        (4,    78.71)
        (8,    92.16)
        };
      \addlegendentry{$h=2^{-8}$}
      \end{axis}
\end{tikzpicture}
\caption{CPU times for different refinement levels with two-level MGRIT and a sequential algorithm for a fixed problem size ($N_t=100,p=2$).}
\label{fig:parallelrefinement}
\end{figure}

\newpage 

In the previous paragraphs, we increased the problem size by considering different refinement levels while the number of time steps was held constant. However, as the MGRIT methods exploits parallelism in the temporal component, increasing the number of time steps might be more benificial. Figure \ref{fig:paralleltime} shows the computational times using a different number of processors for a different number of time steps. Here, the refinement level is kept constant at $h=2^{-6}$. For the considered configurations, the use of a sequential algorithm is still the most efficient, but the difference is around a factor of $2$. 


\begin{figure}[h!]
\centering
  \begin{tikzpicture}[scale=1.0]
    \begin{axis}[nodes near coords={\pgfmathprintnumber[fixed,fixed zerofill,precision=0]{\pgfplotspointmeta}},point meta=rawy,ybar,every node near coord/.append style={rotate=90, anchor=west,font=\tiny},legend columns=1,legend pos=north west, xmin= 0,xmax=30,ymode=log,ymin=1,ymax=10000,ylabel=CPU Time (s),line width=0.25pt,bar width=0.2cm,bar shift=8mm,xticklabels=\emptynodes]
       \addplot[fill=blue!40] plot coordinates 
      {
        (1,    8.88)
        (7,    18.90)
        (13,   44.58)
        (19,   112.60)
       };
      \addlegendentry{B-Euler}
       \addplot[fill=orange!40] plot coordinates 
      {
        (2,    91.63)
        (8,    167.68)
        (14,   342.07)
        (20,   753.65)        
       };
      \addlegendentry{$MGRIT_1$}
       \addplot[fill=green!40] plot coordinates 
      {
        (3,    63.41)
        (9,    117.93)
        (15,   239.80)
        (21,   528.12)
       };
      \addlegendentry{$MGRIT_2$}
      \addplot[fill=red!40] plot coordinates 
      {
        (4,    42.30)
        (10,   81.17)
        (16,   164.66)
        (22,   358.80)
        };
      \addlegendentry{$MGRIT_4$}
      \addplot[fill=black!40] plot coordinates 
      {
        (5,    38.64)
        (11,   78.77)
        (17,   162.17)
        (23,   354.93)
        };
      \addlegendentry{$MGRIT_8$}

      \end{axis}
        \draw (1.45,-0.45)  node{\tiny $N_t=250$};
        \draw (2.85,-0.45)  node{\tiny $N_t=500$};
        \draw (4.25,-0.45)  node{\tiny $N_t=1000$};
        \draw (5.60,-0.45)  node{\tiny $N_t=2000$};
\end{tikzpicture}
\caption{CPU times for MGRIT and a sequential algorithm for a different number of processors and a fixed problem size ($h=2^{-6},p=2$).}
\label{fig:paralleltime}
\end{figure}

To get a clearer idea of the influence on increasing the refinement level and the number of time steps, we vary both parameters. Table \ref{tab:6} shows how the relative difference (compared to the sequential algorithm) changes when adjusting one (or both) of the parameters. Based on these results, increasing the number of time steps seems to be the most beneficial for the MGRIT method. Here, it should be noted that we consider $p=2$ for these numerical experiments. The difference between both methods decreases even further for higher values of $p$. 

% \begin{table}[h]
% \centering
% \begin{tabular}{c|rrr|rrr|}
%   \multicolumn{1}{c|}{}   & \multicolumn{3}{c|}{$N_t=2000$}   & \multicolumn{3}{c|}{$N_t=8000$}    \\  
% 						 & seq. & MGRIT & rel.& seq. & MGRIT  & rel. \\ \hline
% 		$h=2^{-6}$		 & 	$135.23$ & $354.80$     &$2.62$	 & $829.59$   & 	$1528.74$ & $1.84$ \\
% 		$h=2^{-7}$		 & 	$381.31$ & $1239.17$    &$3.25$  & $2321.94$  & 	$4785.21$ & $2.06$ \\
% \end{tabular}
% \caption{Number of two-level or multilevel MGRIT iterations for solving MP-2 when adopting $V$-cycles.}
% \label{tab:6}
% \end{table}

\end{comment}

// Comments (Neumann)


\begin{comment}
The domain $\Omega$ is varied for the different model problems: For the first model problem, referred to as MP-1, we consider the unit square (i.e. $\Omega = [0,1]^2$). As Isogeometric Analysis describes curved geometries more accurately compared to FEM, the second model involves a curved geometry. That is, as MP-2, $\Omega$ is chosen to be a quarter annulus defined in the first quadrant with inner radius of $1$ and an outer radius of $2$. Finally, a multipatch geometry is considered as MP-3. Figure \ref{fig:domain} illustrates the considered spatial domains for all model problems.



\begin{figure}[h]
\begin{tikzpicture}[scale=0.7]
\draw (0,0) -- (4,0) -- (4,4) -- (0,4) -- (0,0);

\draw (8,0) -- (10,0);
\draw (6,4) -- (6,2);
\draw (10,0) arc (0:90:4cm);
\draw (8,0) arc (0:90:2cm);

\draw[dashed] (14,0) -- (14,4);
\draw[dashed] (12,2) -- (16,2);
\draw (12,0) -- (16,0) -- (16,4) -- (12,4) -- (12,0);
\end{tikzpicture}
\caption{Spatial domain $\Omega$ for the model problems MP-1, MP-2 and MP-3.}
\label{fig:domain}
\end{figure}
\subsection*{Implicit time integration}

First, we consider the MGRIT method using both V-cycles and F-cycles for the implicit case (i.e. Backward Euler). At each time step, a linear system of equations has to be solved, which is done by means of a Conjugate Gradient method. Table \ref{tab:neumann1} shows the number of MGRIT iterations for different mesh widths $h$ and approximation orders $p$ of the B-spline basis functions when a two-level method is considered. Here, F-relaxation is applied at all grids of the MGRIT hierarchy. The number of time steps for all configurations equals $100$.

As a two-level method is considered, the number of iterations obtained when considering $V$-cycles is equal to the use of $F$-cycles for all configurations. Furthermore, the number of iterations is constant for all values of $h$, implying MGRIT to be an optimal algorithm with respect to the problem size. For increasing values of $p$, we observe that the number of MGRIT iterations is constant. This is of particular interest, as the convergence rate of standard multigrid methods is known to be dependent on the approximation order $p$ \cite{Gahalaut2013}.  

\begin{table}[h]
\begin{tabular}{c|cccc|cccc|}
  \multicolumn{1}{c|}{}   & \multicolumn{4}{c|}{$V$-cycle}   & \multicolumn{4}{c|}{$F$-cycle}    \\  
             & $p=2$ & $p=3$ & $p=4$ & $p=5$ & $p=2$ & $p=3$ & $p=4$ & $p=5$  \\ \hline
    $h=2^{-4}$     &  $7$  & $7$   & $7$   &  $7$  &  $7$  &  $7$  &  $7$  &   $7$     \\
    $h=2^{-5}$     &  $7$  & $7$   & $7$   &  $7$  &  $7$  &  $7$  &  $7$  &   $7$     \\
    $h=2^{-6}$     &  $8$  & $8$   & $8$   &  $8$  &  $8$  &  $8$  &  $8$  &   $8$     \\
    $h=2^{-7}$     &  $8$  & $8$   & $8$   &  $8$  &  $8$  &  $8$  &  $8$  &   $8$     \\
\end{tabular}
\caption{Number of two-level MGRIT iterations for solving the model problem when adopting $V$-cycle or $F$-cycles.}
\label{tab:neumann1}
\end{table}


Alternatively, a multilevel MGRIT method can be applied as well. Here coarsening is applied with coarsening factor $m=2$, leading to a hierarchy consisting of five levels $(L=5)$. Table \ref{tab:neumann2} shows the number of MGRIT iterations when either $V$-cycles or $F$-cycles are adopted within MGRIT. For all configurations, the use of an $F$-cycle leads to a lower number of MGRIT iterations to reach convergence. However, it should be noted that the computational costs of an $F$-cycle is higher compared to a $V$-cycle. In the next Section, a weak scalability study is preformed using both cycle types.    

\begin{table}[h]
\begin{tabular}{c|cccc|cccc|}
  \multicolumn{1}{c|}{}   & \multicolumn{4}{c|}{$V$-cycle}   & \multicolumn{4}{c|}{$F$-cycle}    \\  
             & $p=2$ & $p=3$ & $p=4$ & $p=5$ & $p=2$ & $p=3$ & $p=4$ & $p=5$  \\ \hline
    $h=2^{-4}$     &  $9$  & $9$   & $9$   &  $9$  &  $7$  &  $7$  &  $7$  &   $7$     \\
    $h=2^{-5}$     &  $9$  & $9$   & $9$   &  $9$  &  $7$  &  $7$  &  $7$  &   $8$     \\
    $h=2^{-6}$     &  $9$  & $9$   & $9$   &  $9$  &  $8$  &  $8$  &  $8$  &   $8$     \\
    $h=2^{-7}$     &  $9$  & $9$   & $9$   &  $9$  &  $8$  &  $8$  &  $8$  &   $8$     \\
\end{tabular}
\caption{Number of two-level MGRIT iterations for solving the model problem when adopting $V$-cycle or $F$-cycles.}
\label{tab:neumann2}
\end{table}

Instead of lowering the meshwidht (and thereby increasing the number of DOF), the number of timesteps can be increased as well. This is in particular interesting as MGRIT is a parallel-in-time method, where speed-ups will primarily come from parallelization in the temporal component. Table \ref{tab:neumann3} shows the number of MGRIT iterations, for a two-level method and when adopting V-cycles for a different number of timesteps and different values of $p$. For all configurations, the use of a two-level MGRIT method leads to a lower number of iterations compared to the use of V-cycles. Note that, the number of iterations are somewhat comparable to the number of iterations obtained when considering different values of the mesh width.

\begin{table}[h]
\begin{tabular}{c|cccc|cccc|}
  \multicolumn{1}{c|}{}   & \multicolumn{4}{c|}{two-level}   & \multicolumn{4}{c|}{multilevel}    \\  
             & $p=2$ & $p=3$ & $p=4$ & $p=5$ & $p=2$ & $p=3$ & $p=4$ & $p=5$  \\ \hline
    $N_t=250$    &  $7$  & $7$   & $7$   &  $7$  &  $10$  &   $10$   &  $10$  &   $10$     \\
    $N_t=500$    &  $7$  & $7$   & $7$   &  $7$  &  $10$  &   $10$   &  $10$  &   $10$     \\
    $N_t=1000$     &  $7$  & $7$   & $7$   &  $7$  &  $11$  &   $11$   &  $11$  &   $11$     \\
    $N_t=2000$     &  $7$  & $7$   & $7$   &  $7$  &  $11$  &   $11$   &  $11$  &   $11$     \\
\end{tabular}
\caption{Number of two-level or multilevel MGRIT iterations for solving MP-2 when adopting $V$-cycles.}
\label{tab:neumann3}
\end{table}

With implicit time integration methods, spatial solves are required at every time step denoted by the function $\Psi$. As these linear systems are solved by means of an iterative method (e.g. Conjugate Gradient), the adopted stopping criterion in these methods (at the coarser levels) might influence the overall convergence of the MGRIT method.   

Table \ref{tab:3} shows the number of MGRIT iterations for different values of the stopping criterion at the coarse levels of the MGRIT hierarchy. Here, $\epsilon$ denotes the norm of the residual divided by the norm of the righthandside and a mesh width is adopted of $h=2^{-6}$. In general, the number of MGRIT is independent of the chosen stopping criterion on the coarser levels. However, when the stopping criterion is chosen too small, the number of MGRIT increases significantly, in particular for smaller values of $p$. 

\begin{table}[h]
\centering
\begin{tabular}{c|cccc}
            & $p=2$ & $p=3$  & $p=4$ & $p=5$  \\ \hline
$\epsilon=10^{-6}$    &   $*$  &  $*$  &  $*$ & $*$  \\
$\epsilon=10^{-8}$    &   $*$  &  $*$  &  $*$  & $*$   \\
$\epsilon=10^{-10}$   &   $9$  &  $83$ &  $*$  & $*$   \\
$\epsilon\approx10^{-16}$&  $9$  &  $9$  &  $9$  & $9$   \\
\end{tabular}
\caption{Number of multilevel MGRIT iterations for solving the model problem (using $V$-cycles) when adopting different stopping criteria at the coarse levels.}
\label{tab:3}
\end{table}


\subsection*{Explicit time integration schemes}
The use of explicit time integration schemes in the context of parallel-in-time integration is on one hand highly relevant, as the required number of time steps needed to ensure stability is relatively high. On the other hand, coarsening with respect to the time step size might still exhibit stability issues at coarser levels. Therefore, explicit-implicit methods are often considered, where explicit time integration is applied on the fine scale problem, while implicit methods are adopted at the coarser levels. 

An obvious drawback of this approach is that one has to implement both time integration schemes within the code. Furthermore, the question remains to which extend the resulting MGRIT algorithm remains robust in the mesh width and/or approximation order. Table \ref{tab:3A} shows the number of two-level MGRIT iterations for different number of time steps when adopting a mesh width of $h=2^{-4}$. Here, explicit Euler is applied at the fine level, while Backward Euler is applied at the coarse level. Note that, provided a small enough time step size is chosen, the resulting MGRIT method convergences is a relatively low number of iterations. However, the higher the approximation order, the lower the time step size has to be chosen to ensure convergence of the MGRIT method. 

\begin{table}[h]
\centering
\begin{tabular}{c|cccc}
        & $p=2$ & $p=3$ & $p=4$  & $p=5$  \\ \hline
$N_t=250$   &   $*$  &  $*$  &  $*$  & $*$   \\
$N_t=500$   &   $13$ &  $*$  &  $*$  & $*$   \\
$N_t=1000$    &   $13$ &  $13$ &  $*$  & $*$   \\
$N_t=2000$    &   $13$ &  $13$ &  $13$ & $*$   \\
\end{tabular}
\caption{Number of two-level MGRIT iterations for solving the model problem (using $V$-cycles) when adopting a different number of time steps. Here, explicit Euler is applied at the fine level, while Backward Euler is applied at the coarse level.}
\label{tab:3A}
\end{table}

Apart from first order time integration methods, MGRIT can be combined with higher-order time integration methods as well. Table \ref{tab:3B} shows the number of two-level MGRIT iterations when the second-order accurate Crank-Nicolson method is applied for the time integration when adopting a mesh width of $h=2^{-4}$. The resulting MGRIT method convergences is a relatively low number of iterations, provided a small enough time step size is chosen.

\begin{table}[h]
\centering
\begin{tabular}{c|cccc}
        & $p=2$ & $p=3$ & $p=4$  & $p=5$  \\ \hline
$N_t=200$   &   $8$  &  $38$ &  $*$  & $*$   \\
$N_t=400$   &   $6$  &  $9$  &  $47$ & $*$   \\
$N_t=600$   &   $6$  &  $6$  &  $8$  & $36$   \\
$N_t=800$   &   $6$  &  $6$  &  $6$  & $7$   \\
\end{tabular}
\caption{Number of two-level MGRIT iterations for solving the model problem (using $V$-cycles) when adopting a different number of time steps. Here, Crank-Nicolson is applied at all levels.}
\label{tab:3B}
\end{table}

\subsection*{Alternative Benchmark problems}

Instead of adopting the unit square as our domain of interest, alternative domains will be considered as well. We consider the MGRIT method applied on curved and multipatch geometries (while using Backward-Euler). Table \ref{tab:neumann4} shows the number of two-level and multilevel MGRIT iterations needed to reach convergence for the heat equation on a quarter annulus (i.e. MP-2). Here, $V$-cycles are applied and results can be compared to Table \ref{tab:neumann3}. In general, results are identical to the ones obtained for MP-1, showing iteration numbers indepedent of the problem size and order of the B-spline basis functions. 



\begin{table}[h]
\begin{tabular}{l|cccc|cccc|}
  \multicolumn{1}{c|}{}   & \multicolumn{4}{c|}{Two-level}   & \multicolumn{4}{c|}{$V$-cycle}    \\  
             & $p=2$ & $p=3$ & $p=4$ & $p=5$ & $p=2$ & $p=3$ & $p=4$ & $p=5$  \\ \hline
    $N_t=250$    &  $7$  & $7$   & $7$   &  $7$  &  $10$  &   $10$   &  $10$  &   $10$     \\
    $N_t=500$    &  $7$  & $7$   & $7$   &  $7$  &  $10$  &   $10$   &  $10$  &   $10$     \\
    $N_t=1000$     &  $7$  & $7$   & $7$   &  $7$  &  $11$  &   $11$   &  $11$  &   $11$     \\
    $N_t=2000$     &  $7$  & $7$   & $7$   &  $7$  &  $11$  &   $11$   &  $11$  &   $11$     \\
\end{tabular}
\caption{Number of two-level MGRIT iterations for solving model problem MP-2 when adopting a two-level method or $V$-cycles.}
\label{tab:neumann4}
\end{table}

Alternatively, the number of time steps can be kept constant ($N_t=100$), while varying the refinement level. Table \ref{tab:neumann5} shows these results for MP-2 when a two-level method and $V$-cycles are adopted. Compared to MP-1 the results are identical for all configurations.  

\begin{table}[h]
\begin{tabular}{l|cccc|cccc|}
  \multicolumn{1}{c|}{}   & \multicolumn{4}{c|}{Two-level}   & \multicolumn{4}{c|}{$V$-cycle}    \\  
             & $p=2$ & $p=3$ & $p=4$ & $p=5$ & $p=2$ & $p=3$ & $p=4$ & $p=5$  \\ \hline
    $h=2^{-4}$     &  $7$  & $7$   & $7$   &  $7$  &  $9$  &  $9$  &  $9$  &   $9$     \\
    $h=2^{-5}$     &  $7$  & $7$   & $7$   &  $7$  &  $9$  &  $9$  &  $9$  &   $9$     \\
    $h=2^{-6}$     &  $8$  & $8$   & $8$   &  $8$  &  $9$  &  $9$  &  $9$  &   $9$     \\
    $h=2^{-7}$     &  $8$  & $8$   & $8$   &  $8$  &  $9$  &  $9$  &  $9$  &   $9$     \\
\end{tabular}
\caption{Number of two-level MGRIT iterations for solving model problem MP-2 when adopting a two-level method or $V$-cycles.}
\label{tab:neumann5}
\end{table}

Table \ref{tab:neumann6} shows the number of two-level and multilevel MGRIT iterations needed to reach convergence for the heat equation on a quarter annulus (i.e. MP-2). Here, $V$-cycles are applied and results can be compared to Table \ref{tab:neumann3}. In general, results are identical to the ones obtained for MP-1, showing iteration numbers indepedent of the problem size and order of the B-spline basis functions. 

\begin{table}[h]
\begin{tabular}{l|cccc|cccc|}
  \multicolumn{1}{c|}{}   & \multicolumn{4}{c|}{Two-level}   & \multicolumn{4}{c|}{$V$-cycle}    \\  
             & $p=2$ & $p=3$ & $p=4$ & $p=5$ & $p=2$ & $p=3$ & $p=4$ & $p=5$  \\ \hline
    $N_t=250$    &  $7$  & $7$   & $7$   &  $7$  &  $10$  &   $10$   &  $10$  &   $10$     \\
    $N_t=500$    &  $7$  & $7$   & $7$   &  $7$  &  $10$  &   $10$   &  $10$  &   $10$     \\
    $N_t=1000$     &  $7$  & $7$   & $7$   &  $7$  &  $11$  &   $11$   &  $11$  &   $11$     \\
    $N_t=2000$     &  $7$  & $7$   & $7$   &  $7$  &  $11$  &   $11$   &  $11$  &   $11$     \\
\end{tabular}
\caption{Number of two-level MGRIT iterations for solving model problem MP-3 when adopting a two-level method or $V$-cycles.}
\label{tab:neumann6}
\end{table}

Alternatively, the number of time steps can be kept constant ($N_t=100$), while varying the refinement level. Table \ref{tab:neumann7} shows these results for MP-3 when a two-level method and $V$-cycles are adopted. Compared to MP-1 the results are identical for all configurations.  

\begin{table}[h]
\begin{tabular}{l|cccc|cccc|}
  \multicolumn{1}{c|}{}   & \multicolumn{4}{c|}{Two-level}   & \multicolumn{4}{c|}{$V$-cycle}    \\  
             & $p=2$ & $p=3$ & $p=4$ & $p=5$ & $p=2$ & $p=3$ & $p=4$ & $p=5$  \\ \hline
    $h=2^{-4}$     &  $7$  & $7$   & $7$   &  $7$  &  $9$  &  $9$  &  $9$  &   $9$     \\
    $h=2^{-5}$     &  $7$  & $7$   & $7$   &  $7$  &  $9$  &  $9$  &  $9$  &   $9$     \\
    $h=2^{-6}$     &  $7$  & $7$   & $7$   &  $7$  &  $9$  &  $9$  &  $9$  &   $9$     \\
    $h=2^{-7}$     &  $8$  & $8$   & $8$   &  $8$  &  $9$  &  $9$  &  $9$  &   $9$     \\
\end{tabular}
\caption{Number of two-level MGRIT iterations for solving model problem MP-3 when adopting a two-level method or $V$-cycles.}
\label{tab:neumann7}
\end{table}

\newpage

\subsection{Parallel performance}

To investigate the parallel performance of the MGRIT method, CPU times have been obtained using a different number of processors. Here, we consider three computational nodes, each consisting of $8$ CPU's (Intel i7 ... gHZ). 

Figure \ref{fig:paralleltime_neumann1} shows the obtained CPU times for a sequential time-integration scheme (Backward-Euler), a two-level method, V-cycles and F-cycles when considering a different number of time steps. Here, we consider model problem MP-1, a mesh width of $h=2^{-6}$ and an approximation order of $p=3$. Clearly, the use of a traditional sequential time-integration scheme leads to the lowest CPU times for all configurations. When comparing the different multigrid hierarchies, the two-level method is most efficient and will therefore be adopted when further investigating the parallel performance of MGRIT.    

\begin{figure}[h!]
\centering
  \begin{tikzpicture}[scale=1.0]
    \begin{axis}[nodes near coords={\pgfmathprintnumber[fixed,fixed zerofill,precision=0]{\pgfplotspointmeta}},point meta=rawy,ybar,every node near coord/.append style={rotate=90, anchor=west,font=\tiny},legend columns=4,legend pos=north west, xmin= 0,xmax=30,ymode=log,ymin=1,ymax=10000,ylabel=CPU Time (s),line width=0.25pt,bar width=0.2cm,bar shift=8mm,xticklabels=\emptynodes]
       \addplot[fill=blue!40] plot coordinates 
      {
        (1,    3.58)
        (7,    7.33)
        (13,   15.69)
        (19,   35.57)
       };
      \addlegendentry{BE}
       \addplot[fill=orange!40] plot coordinates 
      {
        (2,    26.08)
        (8,    47.99)
        (14,   92.56)
        (20,   186.03)        
       };
      \addlegendentry{Two-Level}
       \addplot[fill=green!40] plot coordinates 
      {
        (3,    57.21)
        (9,    109.38)
        (15,   234.04)
        (21,   467.98)
       };
      \addlegendentry{V-cycle}
      \addplot[fill=red!40] plot coordinates 
      {
        (4,    78.51)
        (10,   153.37)
        (16,   297.22)
        (22,   594.38)
        };
      \addlegendentry{F-cycle}
      \end{axis}
        \draw (1.45,-0.45)  node{\tiny $N_t=250$};
        \draw (2.85,-0.45)  node{\tiny $N_t=500$};
        \draw (4.25,-0.45)  node{\tiny $N_t=1000$};
        \draw (5.60,-0.45)  node{\tiny $N_t=2000$};
\end{tikzpicture}
\caption{CPU times for different variants of MGRIT for $3$ processors and a fixed problem size ($h=2^{-6},p=3$) compared to a sequential Backward Euler (BE) method.}
\label{fig:paralleltime_neumann1}
\end{figure}



\begin{figure}[h!]
\centering
  \begin{tikzpicture}[scale=1.0]
    \begin{axis}[nodes near coords={\pgfmathprintnumber[fixed,fixed zerofill,precision=0]{\pgfplotspointmeta}},point meta=rawy,ybar,every node near coord/.append style={rotate=90, anchor=west,font=\tiny},legend columns=5,legend pos=north west, xmin= 0,xmax=30,ymode=log,ymin=1,ymax=1000,ylabel=CPU Time (s),line width=0.25pt,bar width=0.2cm,bar shift=8mm,xticklabels=\emptynodes]
       \addplot[fill=blue!40] plot coordinates 
      {
        (1,    3.58)
        (7,    7.33)
        (13,   15.69)
        (19,   35.57)
       };
      \addlegendentry{BE}
       \addplot[fill=orange!40] plot coordinates 
      {
        (2,    26.08)
        (8,    47.99)
        (14,   92.56)
        (20,   186.03)        
       };
      \addlegendentry{$n_p=3$}
       \addplot[fill=green!40] plot coordinates 
      {
        (3,    19.69)
        (9,    37.35)
        (15,   71.29)
        (21,   141.41)
       };
      \addlegendentry{$n_p=6$}
      \addplot[fill=red!40] plot coordinates 
      {
        (4,    15.63)
        (10,   31.20)
        (16,   62.48)
        (22,   123.25)
        };
      \addlegendentry{$n_p=12$}
      \addplot[fill=black!40] plot coordinates 
      {
        (5,    14.37)
        (11,   32.08)
        (17,   64.58)
        (23,   130.17)
        };
      \addlegendentry{$n_p=24$}

      \end{axis}
        \draw (1.45,-0.45)  node{\tiny $N_t=250$};
        \draw (2.85,-0.45)  node{\tiny $N_t=500$};
        \draw (4.25,-0.45)  node{\tiny $N_t=1000$};
        \draw (5.60,-0.45)  node{\tiny $N_t=2000$};
\end{tikzpicture}
\caption{CPU times for MGRIT for a different number of processors and a fixed problem size ($h=2^{-6},p=3$) compared to a sequential Backward Euler (BE) method.}
\label{fig:paralleltime_neumann}
\end{figure}
\end{comment}


